Comprehensive Optimization of Parametric Kernels for Graphics Processing Units

This work deals with the optimization of computer programs targeting Graphics Processing Units (GPUs). The goal is to lift, from programmers to optimizing compilers, the heavy burden of determining program details that are dependent on the hardware characteristics. The expected benefit is to improve robustness, portability and efficiency of the generated computer programs. We address these requirements by: (1) treating machine and program parameters as unknown symbols during code generation, and (2) generating optimized programs in the form of a case discussion, based on the possible values of the machine and program parameters. By taking advantage of recent advances in the area of computer algebra, preliminary experimentation yield promising results.

==> MD-example-2-columns.tex <==
\ifextendedabstract
We conclude this extended abstract with an example
illustrating 
\else
Let us illustrate, with an example, 
\fi
the notion of comprehensive
parametric {\cuda} kernels, along with a procedure to generate them.
Our input is the for-loop nest of Figure~\ref{fig:tiledmetaforloop}
 which
computes the sum of two matrices {\tt b} and {\tt c} of order $N$
using a blocking strategy; each matrix is divided into
blocks of format ${\tt B0} \times {\tt B1}$.
%%
This input code is 
annotated for parallel execution in the {\meta} language.
The body of the statement \textcolor{red}{\tt meta\_schedule} is meant
to be offloaded to a GPU device and each
\textcolor{red}{meta\_for} loop is a parallel for-loop
where all iterations can be executed concurrently.
%%

\begin{figure}[!htb]
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\footnotesize]
  int dim0 = N/B0, dim1 = N/(2*B1);
  \textcolor{red}{meta_schedule} \{
    \textcolor{red}{meta_for} (int v = 0; v < dim0; v++)
      \textcolor{red}{meta_for} (int p = 0; p < dim1; p++)
        \textcolor{red}{meta_for} (int u = 0; u < B0; u++) 
          \textcolor{red}{meta_for} (int q = 0; q < B1; q++) \{
            int i = v * B0 + u;
            int j = p * B1 + q;
            if (i < N && j < N/2) \{
              c[i][j] = a[i][j] + b[i][j]; 
              c[i][j+N/2] = 
                 a[i][j+N/2] + b[i][j+N/2]; 
            \}
          \}
  \}
\end{Verbatim}
\caption{A \textcolor{red}{\tt meta\_for} loop nest for adding two matrices.}
\label{fig:tiledmetaforloop}
\end{figure}


We make the following simplistic assumptions for the 
translation of this for-loop nest to {\cuda}.
\begin{enumerateshort}
\item The target machine has two parameters: the maximum number $R$ 
      of registers per thread, and the maximum number $T$ of threads per 
      thread-block; all other hardware limits are ignored.
\item The generated kernels depend on two program parameters, $B_0$ and
      $B_1$, which define the format of a 2D thread-block.
\item The optimization strategy (w.r.t. register usage per thread) 
      consists in reducing the work per thread
      (by reducing loop granularity).
\end{enumerateshort}
A possible comprehensive parametric {\cuda} kernel 
is given by the pairs $(C_1, K_1)$ and $(C_2, K_2)$, where $C_1, C_2$ are
two sets of algebraic constraints on the parameters and $K_1, K_2$ are
two {\cuda} kernels that are optimized under the 
constraints respectively given by $C_1, C_2$, 
see Figure~\ref{fig:compparkern}.
%%
The following computational steps yield the 
pairs $(C_1, K_1)$ and $(C_2, K_2)$.
%%
\begin{enumerateshort}
%%
\item[(S1)]  The {\meta} code is mapped to an
      intermediate representation (IR)
      say that of {\llvm}\footnote{
       Quoting Wikipedia: 
       ``The {\llvm} compiler infrastructure project 
       (formerly Low Level 
       Virtual Machine~\cite{Lattner:2004:LCF:977395.977673,Bertolli:2014:CGT:2688361.2688364})
       is a framework for developing 
       compiler front ends and back ends''.}, or alternatively, to
       {\ptx}\footnote{The {\em Parallel Thread Execution} 
       (PTX)~\cite{ptx2015}
        is the pseudo-assembly language to which
       {\cuda} programs are compiled by NVIDIA's {\nvcc} compiler.
       {\ptx} code can also be generated from (enhanced) {\llvm} IR,
       using {nvptx} back-end~\cite{nvptx},
       following the work of~\cite{Rhodin2010}.} code.
%%
\item[(S2)] Using this IR (or {\ptx}) code, one {\em estimates} the 
      number of registers that a thread requires;
     on this example, using {\llvm} IR, we obtain an estimate of $14$.
%%
\item[(S3)] Next, we apply the optimization strategy, yielding 
      a new IR (or {\ptx}) code, for which register pressure reduces to $10$.
      Since no other optimization techniques are considered,
      the procedure stops with the result shown on 
      Figure~\ref{fig:compparkern}.
%%
\end{enumerateshort}
Note that, strictly speaking, the kernels $K_1$ and $K_2$ on
Figure~\ref{fig:compparkern} should be given by {\ptx} code.  But for
simplicity, we are presenting them by counterpart {\cuda} code.


\begin{figure}[!htb]
%%
\begin{minipage}[t]{0.5\textwidth}

\begin{small}
$C_1 : \left\{ \begin{array}{l} B_0 \times B_1 \leq T \\ 14 \leq R \end{array} \right.   $ 
\end{small}

\begin{scriptsize}
\begin{verbatim}
__global__  void K1(int *a, int *b, int *c, int N, 
                                 int B0, int B1) {
     int i = blockIdx.y * B0 + threadIdx.y;
     int j = blockIdx.x * B1 + threadIdx.x;
     if (i < N && j < N/2) {
        a[i*N+j] = b[i*N+j] + c[i*N+j];
        a[i*N+j+N/2] = b[i*N+j+N/2] + c[i*N+j+N/2];
     }
}
dim3 dimBlock(B1, B0);
dim3 dimGrid(N/(2*B1), N/B0);
K1 <<<dimGrid, dimBlock>>> (a, b, c, N, B0, B1);
\end{verbatim}
\end{scriptsize}

\end{minipage}
\begin{minipage}[t]{0.5\textwidth}

\begin{small}
$C_2 : \left\{ \begin{array}{l} B_0 \times B_1 \leq T \\ 10 \leq R < 14 \end{array} \right.  $
\end{small}

\begin{scriptsize}
\begin{verbatim}
__global__  void K2(int *a, int *b, int *c, int N, 
                                 int B0, int B1) {
     int i = blockIdx.y * B0 + threadIdx.y;
     int j = blockIdx.x * B1 + threadIdx.x;
     if (i < N && j < N)
        a[i*N+j] = b[i*N+j] + c[i*N+j];
}
dim3 dimBlock(B1, B0);
dim3 dimGrid(N/B1, N/B0);
K2 <<<dimGrid, dimBlock>>> (a, b, c, N, B0, B1);
\end{verbatim}
\end{scriptsize}
\end{minipage}

\caption{A comprehensive parametric {\cuda} kernel for matrix addition.}
\label{fig:compparkern}
\end{figure}

\ifextendedabstract
While this was a {\em toy-example}, advanced
test cases can be found in Chapter 7 of the PhD thesis
of the first author at
\begin{center}
\url{http://ir.lib.uwo.ca/etd/4429}
\end{center}
\else
This paper is organized as follows.  In
Section~\ref{sec:parametric_kernels}, we review the notion of a {\em
parametric {\cuda} kernel} through an example.
%%
In Section~\ref{sec:comprehensive_optimization},
we introduce the notion of {\em comprehensive optimization}
of a code fragment together with an algorithm for computing it.
%%
In Section~\ref{comprehensive_translation}, we explain
how this latter notion applies to the generation
of parametric {\cuda} kernels generated from 
a program written in  a high-level accelerator model namely
{\meta}.
%%
Finally, experimental results are provided in
Section~\ref{sec:experimentation}.
\fi

